Integrating AI in NDE: Techniques, Trends, and Further Directions

The digital transformation is fundamentally changing our industries, affecting planning, execution as well as monitoring of production processes in a wide range of application fields. With product line-ups becoming more and more versatile and diverse, the necessary inspection and monitoring sparks significant novel requirements on the corresponding Nondestructive Evaluation (NDE) systems. The establishment of increasingly powerful approaches to incorporate Artificial Intelligence (AI) may provide just the needed innovation to solve some of these challenges. In this paper we provide a comprehensive survey about the usage of AI methods in NDE in light of the recent innovations towards NDE 4.0. Since we cannot discuss each NDE modality in one paper, we limit our attention to magnetic methods, ultrasound, thermography, as well as optical inspection. In addition to reviewing recent AI developments in each field, we draw common connections by pointing out NDE-related tasks that have a common underlying mathematical problem and categorizing the state of the art according to the corresponding sub-tasks. In so doing, interdisciplinary connections are drawn that provide a more complete overall picture.

==> sections/SyntheticUS.tex <==

\subsection{Synthetic ultrasound data} \label{sec:ut_datasynth} 

\han{(9 references in 3.5)}

The generation of synthetic data increasingly attracts interest in \gls{ndt} applications such as \gls{ut}. On one hand, the validation of inspection procedures through sizing and classification of defects as well as \gls{pod} requires large amounts of measurement data representing various types of inspection modalities and defects \citep{virkkunen2023virtual}. On the other, the training of \gls{ml} models requires volumes of labeled data pertaining to a particular application which in practice are difficult to obtain. In this section, the augmentation and synthetic generation of measurement data via \gls{ai} is addressed.



In order to study the uncertainty quantification for deep learning in ultrasonic crack characterization, Pyle et al. \citep{PHA22} used a \gls{cnn} architecture to size surface breaking defects from \gls{pwi} images with two modern UQ methods, deep ensembles and Monte Carlo dropout. The network is trained using \gls{pwi} images of surface-breaking defects simulated with a hybrid \gls{fe} / ray-based model. The calibration is tested using simulated and experimental images of surface-breaking cracks, while anomaly detection is tested using experimental side-drilled holes and simulated embedded cracks. Synthetic data is created by a hybrid \gls{fe}/ray-based simulation method. For the training data, 14343 simulated images were used, while the validation data consisted of 1266 simulated and 216 experimental images, and the test data was given by 1266 simulated and 216 experimental images. They found, that "Monte Carlo dropout demonstrates poor uncertainty quantification with little separation between in and out-of-distribution data and a weak linear fit (\gls{cor} = 0.84) between experimental root-mean-square-error and uncertainty. Deep ensembles improve upon Monte Carlo dropout in both calibration (\gls{cor} = 0.95) and anomaly detection. Adding spectral normalization and residual connections to deep ensembles slightly improves calibration (\gls{cor} = 0.98) and significantly improves the reliability of assigning high uncertainty to out-of-distribution samples." Another work dealing with crack detection is given by Gantala et al. \citep{GB21}, who generated synthetic \gls{tfm} imaging datasets by \gls{fem} simulation as well as by use of a \gls{gan} to develop an \gls{adr} in butt-welds. They constructed six types of imaging datasets: 1. weld \gls{tfm} images are constructed using \gls{us} A-scan signals from \gls{fmc} (using \gls{fe} analysis on models with weld defects); 2. real-time weld \gls{tfm} images by implementing fast \gls{dcgan}; and 3. in order to create near to realistic scenarios, noise is extracted from \gls{fmc}-\gls{tfm} experimental measurements using the sliding kernel approach, and this noise is supplemented to individual simulated datasets; 4.-6. in addition, three further data sets were generated by combining these methods.  To classify and detect the weld defects in an image a pre-trained YOLOv4 network was finetuned. With their approach, they were able to achieve a \SI{100}{\%} \gls{pod} on defect detection and < \SI{10}{\%} on false-calls for the hybrid dataset without noise. However, for the hybrid dataset with noise they achieved \SI{90}{\%} \gls{pod} on defect detection and < \SI{17}{\%} on false-calls. Also, Posilovic et al. \citep{PMS22} used \glspl{gan} in order to generate ultrasonic images indistinguishable from real images. They build up their dataset by scanning six steel blocks containing artificially created defects in the internal structure. The blocks varied in size and contained between six and 34 defects. There were 68 different defects in total. For the ultrasonic acquisition a phased array probe was used. Annotated images were cut into patches of size 256x256 pixels. Finally, there were 3825 images with a total of 6238 annotations. From this dataset, defects in the form of the rectangle patches from the annotations were copied and pasted on \gls{ut} B-scans without defects. There were 3400 empty \gls{ut} images from all of the blocks. Extracted defects that were not extracted well were manually filtered out, such that 4283 defect patches were obtained. They tested three different methods for generating synthetic images. Two of them involve a deep learning approach using a \gls{gan} and one describes a more traditional copy/paste approach. The \gls{gan}-approaches use a binary position mask (256x256 pixels) as input and generate B-scan as output. The first \gls{gan} approach is a detectionGAN model based upon the pix2pixHD, it consists of a U-Net generator with skip connections and two PatchGAN discriminators that work on different scales. It utilizes a pretrained YOLOv3 object detector as an additional discriminator. The second \gls{gan} method is SPADE GAN, which is also based on pix2pixHD with the addition of the encoder for generating noise for the input to the generator. This is done by modifying the architecture by adding the pretrained YOLOv3 discriminator. In order to evaluate proposed methods a test with highly trained human experts was performed.
But also other interesting applications of generative AI in ultrasound applications, for example, Singh et al. \citep{STC22} studied the real-time super-resolution mapping of locally anisotropic grain orientations for ultrasonic non-destructive evaluation of crystalline material. They proposed a framework that makes use of a \gls{dnn} with full aperture, pitch-catch and pulse-echo transducer configurations, to reconstruct material maps of crystallographic orientation. They also presented the application of a \gls{gan} to achieve super-resolution of ultrasonic tomographic images. For the \gls{gan}, the used generator had a U-Net architecture while the discriminator used a PatchGAN architecture. To solve the tomographic inverse problem, a large data set of simulated material maps and corresponding travel time measurements was used to train the network. With their approach, they achieved a factor-four increase in image resolution and up to a $\SI{50}{\%}$ increase in structural similarity. Another interesting work was given by by Ni et al. \citep{NG20}, they tackled the inverse problem of modulus identification in elasticity with a generative deep learning approach. They constructed representative sampling spaces of shear modulus distribution and adopted a conditional generative adversarial net. For the generation of modulus images, a strain image was used as input for the cGAN generator which was based on an unet architecture. Discrimination was carried out by using a PatchGan classifier, which gets pairs of modulus and strain images as inputs.

%-----------------------------------------
% FW problem approach: FEMs and PINNs
Since ultrasound propagation obeys physical laws, solving wave equations \eqref{eq_wave} is another approach for \gls{ut} data synthesization. Conventionally, \glspl{pde} including wave equations are solved using classical numerical methods such as finite elements or spectral approaches \citep{GB21, PHA22}. Due to their robustness and sophisticated algorithms, such numerical methods play crucial roles when it comes to data synthesization. Yet, their high computational cost may become prohibitive especially when dealing with a large 3D region. Since the object surface needs to be specified, dealing with a complicated geometry is also challenging with such numerical methods. \par

In this regard, \glspl{pinn} are beneficial and can complement the existing numerical methods \citep{raissi2019physics}. 
%By constraining the network to satisfy the \gls{pde} of interest, \glspl{pinn} respect the underlying physics while exploiting the powerful computation capability of \glspl{nn}. Compared to vanilla type of \glspl{nn}, \glspl{pinn} can be trained effectively with small data sets as they only require few samples from the boundary and the initial points. \glspl{pinn} can be constructed mesh-free, overcoming the curse of dimensionality one faces with classical numerical methods. Its implementation simplicity eases its use with complicated geometries as well. Furthermore, the successfully trained network is a direct functional approximation of the \gls{pde} of interest, which can be used for solving both forward and inverse problems. For further details on \gls{pinn}, we refer to the comprehensive review given in \citep{Karniadakis21pinnreview}. \par
% For solving wave equation
% Moseley
Specifically for solving wave equations, there exist several approaches. The effectiveness of \gls{pinn} is showcased in \citep{moseley2020solving} where a simple shallow \gls{mlp} with 10 layers suffices to simulate 2D wave propagation even in an inhomogeneous medium. 
% Song: Helpholtz + PML
Another work \citep{Song2021pinnhelmholtz} addresses the difficulty in balancing the physics and the boundary loss by modeling the boundaries as perfectly matched layers and integrating them into the Helmholtz equation \eqref{eq_helm}. Though it works only for absorbing boundaries, i.e. when the region of interest is sufficiently distanced from any boundaries, the trained \gls{pinn} demonstrates remarkable performance in inferring 2D wave fields in inhomogeneous media with anisotropic wave speed. 
% Offen: variational 
The wave equation can be also solved in the variational form, and its adaptation to \gls{pinn} presents successful inference of 1D wave propagation in a homogeneous medium with reflective boundaries \citep{Offen2023pinnvariational}. With the variational form, a second order \gls{pde} is reformulated as a first-order differential equation of the underlying action functional, making it an effective alternative for solving the wave equation in the time domain.
% Further detail
For further details and a general overview of \gls{pinn}, we refer to the comprehensive review given in \citep{Karniadakis21pinnreview}. 

\red{for reference, the whole ultrasound section is roughly 8 pages long, magnetic inspection one is about 6, and thermography and optical inspection are 3 and 2, respectively. That means ultrasound and magnetic methods might be places to save space if we have issues with the page limit.}


==> sections/model_based_DL.tex <==

\subsubsection{Ultrasonic Imaging with Model-Based Deep Learning} \label{model_based_DL}
%begin{itemize}
%    \item deep algorithm unfolding
%    \item[-] Linear layers --> Multilayer Perception 
%    \item[-] Convolutional layers --> CNN 
%    \item[*] Raw data (combined A-scan) 
%    \item[*] Beamforming <-- model-based deep learning --> deep generative AI (adaptive sensing)
%\end{itemize}

\han{(35 references in 3.1.2, Han will reduce some of them)}

In conventional ultrasound signal processing, leveraging prior knowledge, such as known data structures and underlying physics, plays a pivotal role \citep{drinkwater2006ultrasonic}. Model-based algorithms utilizing domain knowledge have been developed, such as those employing message passing in ultrasound imaging \citep{kim2016ultrasound}. While these classical methods are interpretable, they heavily rely on specific domain knowledge. In contrast, purely data-driven approaches attempt to solve similar problems by harnessing the vastness of available data \citep{liu2019deep, van2019deep}. Deep learning technologies, adaptable to various scenarios, are particularly valuable in the absence of specific domain knowledge. However, deep learning requires substantial datasets, and its black-box nature limits explainability. To merge the strengths of model-based algorithms and deep learning, the concept of \emph{model-based deep learning} has recently emerged \citep{shlezinger2022model}.

Model-based deep learning integrates prior models into \glspl{dnn}, a concept that, although formalized recently, has roots dating back more than a decade. The seminal work by \citep{gregor2010learning} in 2010 replaced standard iterations in \gls{ista} with neural network layers, birthing the \gls{lista} algorithm for sparse signal recovery, marking an early instance of model-based deep learning applications. A recent comprehensive survey \citep{shlezinger2023model} delves into model-based deep learning, offering insights into concepts, design strategies, and applications. The survey categorizes model-based deep learning into two main types: \emph{model-aided networks}, which integrate complete \glspl{dnn} with standard model-based algorithms, such as \emph{deep unfolding} or \emph{algorithm unrolling} \citep{hershey2014deep, monga2021algorithm}; and \emph{\gls{dnn}-aided inference}, which replaces parts of the original approach with \glspl{dnn}. The architecture of deep unfolding networks is illustrated in \cref{fig_unfolding}. As an example of \gls{dnn}-aided inference, \citep{bora2017compressed} leverages generative models to map a lower-dimensional vector to an approximation of the sparse signal $\boldsymbol{\gamma}$, aiding subsequent optimization processes.

Beamforming, a cornerstone in ultrasound imaging, has witnessed significant advancements through the application of standard \gls{ai} techniques. In a pivotal study by Hyun et al. \citep{hyun2019beamforming}, a fully \gls{cnn} was leveraged for beamforming, surpassing existing speckle reduction methods. In the realm of compressed beamforming \citep{chernyakova2014fourier}, Khan et al. \citep{khan2020adaptive} introduced a groundbreaking \gls{dnn} capable of processing both full and subsampled \emph{radio frequency} data. This innovative approach generated high-quality images using a single beamformer. Additionally, their study introduced a \gls{cnn} trained on sub-Nyquist sampled and spatially subsampled channel data, mastering the transformation to produce high-quality B-mode images \citep{mamistvalov2022deep}. Notably, Nair et al. \citep{nair2018deep} proposed a \gls{cnn} framework that reimagined traditional beamforming as a segmentation problem, thereby eliminating the need for multiple insonification angles. Building on this foundation, their subsequent work \citep{nair2020deep} delved deeper into the potential of \glspl{dnn} as an alternative to \gls{das} beamforming. This exploration aimed at extracting information directly from raw channel data, simultaneously generating a segmentation map for automated tasks and a B-mode image for interpretable supervision.

Moreover, the integration of model-based deep learning into beamforming has emerged as a promising frontier. Van et al. \citep{van2021deep} pioneered the incorporation of Deep Learning methods into ultrasound imaging, enhancing image reconstruction across various scanning modes, digital receive beamforming techniques, network architectures, and training approaches. In a parallel effort, Luijten et al. \citep{luijten2023ultrasound} endeavored to bridge the chasm between conventional ultrasound signal processing and model-based deep learning. Their work shed light on the transformation of beamforming into parameter estimation problems, demonstrating how classic methods such as \gls{das} and \gls{mv} beamforming could be reformulated as \emph{maximum likelihood} solutions under white and colored Gaussian noise. Specifically, Luijten introduced a model-based \gls{dnn} rooted in principles of \gls{mv} beamforming, facilitating high-quality image reconstruction while significantly reducing computational time \citep{luijten2019deep}. Furthermore, he proposed a distinctive method known as \gls{able}, outlined in his work \citep{luijten2020adaptive}, which empowers the generation of high-quality images through a relatively compact model-based neural network.

In the realm of model-based deep learning approaches, deep unfolding stands out as one of the most prevalent methods, primarily owing to its transparency, reliability, and simplicity, as noted in the work of Li et al. (2021) \citep{li2021deep}. This technique, rooted in the established \gls{admire} approach introduced by Byram et al. (2015) \citep{byram2015model}, has demonstrated its efficacy in enhancing image quality by effectively suppressing acoustic clutter, as evidenced by the studies conducted by Khan and colleagues (2021, 2022) \citep{khan2021performing, khan2022unfolding}. Within the specific domain of \gls{ceus}, an innovative model-based \gls{dnn} named \gls{corona} has been proposed. \gls{corona} represents a pioneering approach where the iterative algorithm is meticulously unfolded into a fixed-length architecture. This unfolding process significantly contributes to the improvement of both convergence and image quality, thereby advancing the field \citep{solomon2019deep}.

Moreover, the integration of model-based deep learning techniques within the framework of \gls{cs} is particularly noteworthy. This integration enables the exploration of optimal subsampling patterns, showcasing the remarkable versatility and adaptability of model-based deep learning in diverse contexts. Specifically, assuming that the beamformed signal generated by frequency-domain beamforming \citep{chernyakova2014fourier} or \gls{coba} \citep{cohen2018sparse} adheres to a \gls{fri} structure, an efficient model-based \gls{dnn} incorporating a modified version of \gls{lista} is employed. This approach significantly reduces the number of array elements, sampling rate, and computational time, as demonstrated by Mamistvalov et al. \citep{mamistvalov2021deep}. Furthermore, Huijben applied the Gumbel-Softmax reparameterization trick to \gls{lista}, introducing the \gls{dps} approach \citep{huijben2020learning}. Within the \gls{dps} framework of model-based deep learning, an optimal spatial subsampling design for single-channel synthetic aperture imaging is introduced. This design is based on the dual objectives of maximizing Fisher information \citep{wang2023smsi} and minimizing reconstruction error \citep{wang2023eusipco}. Additionally, this approach is extended to the field of phased array ultrasound nondestructive testing. Here, it efficiently selects optimal transmitters, receivers, and sampled Fourier coefficients during measurements \citep{wang2023ius}. This remarkable combination of techniques not only enhances the efficiency of subsampling but also contributes significantly to the advancement of various applications in the realm of signal processing and imaging. %\citep{vishnevskiy2018image, bernhardt2020training, chennakeshava2020high, ahmadi2022photothermal}.
\begin{figure}[ht!]
	\centering
	\includegraphics[width=0.8\columnwidth, trim = {0cm 0cm 0cm 0cm}, clip]{images/J-DPS_network.eps}
	\caption{Structure of Joint DPS Algorithm \han{(WIP: add ICASSP reference and text to explain this figure)}}
	\label{fig_jdps}
\end{figure}

==> sections/optische_pr__fung.tex <==
\section{Optical Inspection} \label{opt._insp.}

A significant fraction of \gls{ndt} tasks can be solved through optical inspection methods, i.e., based on optical sensors using image processing methods. Such optical systems can consist of cameras, lasers, scanners, or a combination of the above. However, machine vision with a camera is the most common. \Cref{fig:camsys} shows the typical workflow of a camera system for optical inspection \citep{9214824}.
\begin{figure} [h]
  \centering
  \begin{tikzpicture}[>=stealth, node distance=1 cm]

    % Nodes
    \node (item) [draw, rectangle] {Test Specimen};
    \node (ki) [draw, rectangle, below of=item] {Camera \& Illumination};
    \node (computer) [draw, rectangle, below of=ki] {Computer};
    %\node (imageacq) [draw, rectangle, right of=computer, xshift=2cm] {Image Acquisition};
    \node (feature) [draw, rectangle, below of=computer] {Feature Extraction};
    \node (classification) [draw, rectangle, below of=feature] {Classification};
    \node (controller) [draw, rectangle, below of=classification] {Controller};

    % Arrows
    \draw[->] (item) -- (ki);
    \draw[->] (ki) -- (computer) node[midway, right] {Image Acquisition};
    \draw[->] (computer) -- (feature);
    %\draw[->] (imageacq) -- (feature);
    \draw[->] (feature) -- (classification);
    \draw[->] (classification) -- (controller);

  \end{tikzpicture}
  \caption{Setup of a camera system}
  \label{fig:camsys}
\end{figure}

A camera and a suitable (active or passive) illumination are used to take one or multiple images of the specimen, which are subsequently transferred to the computer. 
The image matrix $\bm{P}$ for a grayscale image can be represented as $m \times n$ matrix where each entry $\bm{P}(i, j)$ represents the brightness value of the pixel located at the $i$-th row and $j$-th column of the image.
Afterwards, feature extraction is applied. Feature extraction in an image can be mathematically represented as a function $f(\bm{P})$ that transforms the original image into a set of features or vectors:
\begin{equation}
    f(\bm{P}) = \{\bm{f}_1, \bm{f}_2, \ldots, \bm{f}_k\}
\end{equation}
Here, $\bm{f}_1, \bm{f}_2, \ldots, \bm{f}_k$ represent the extracted features. These features can be of various types, depending on the type of analysis.
Then the data can be classified. The classification process can be mathematically represented as a function $c(f(\bm{P}))$ that maps the features to a specific class or label:
\begin{equation}
    c(f(\bm{P})) \in \mathcal{C}
\end{equation}
Here, $\mathcal{C}$ is the set of all classes under consideration, and $c$ yields a class or label for the image or region based on the extracted features. After the data evaluation, the process chain ends with a controller, which makes a certain decision depending on the class.\\

Nowadays, thanks to the advanced development of neural networks, many of these problems can be solved via Deep Learning. A simple scheme is shown in  \Cref{fig:cnn_architecture}.

\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        % Input layer
        \node[rectangle split, rectangle split parts=2, draw, align=center] (input) {
            \textbf{Input Layer}
            \nodepart{two} Input Image
        };

        % Convolutional layer
        \node[rectangle split, rectangle split parts=4, draw, right=0.4cm of input, align=center] (conv) {
            \textbf{Hidden Layer}
            \nodepart{two} Convolutional
            \nodepart{three} Pooling
            \nodepart{four} Fully Connected
        };

        % Output layer
        \node[rectangle split, rectangle split parts=2, draw, right=0.4cm of conv, align=center] (output) {
            \textbf{Output Layer}
            \nodepart{two} Predicted Classes
        };

        % Arrows

        \draw[->] (input) -- (conv);

        \draw[->] (conv) -- (output);

    \end{tikzpicture}
    \caption{Convolutional Neural Network (CNN) Architecture}
    \label{fig:cnn_architecture}
\end{figure}

In the example, the input image goes through many different convolution operations, a common approach in image processing to establish shift invariance of detected objects across the image. During this process, corresponding feature maps are created. The feature maps are compressed by the pooling layer. The fully connected layer connects the different maps so that the desired classification is obtained in the end.

Overall, there are countless examples from the field of visual inspection \citep{see2017role}, which can benefit from AI. As an illustrative example, we introduce the task of corrosion detection. It can be considered representative for many optical inspection tasks.  

\subsection{Image Processing-Based Corrosion Detection}
\label{img-based-corro-detec}

Corrosion detection is a practical example of optical inspection. Whether bridges, ancillary structures for highways, piers and other such structures, it is essential to inspect them regularly for corrosion. This inspection is often still performed by people visually. However, this is very time-consuming and costly. For this reason, Das et. al proposed the automated detection of corrosion by means of image processing \citep{infrastructures8040066}.

As usual with conventional image processing, image enhancement was performed at the beginning. In the first step, a contrast adjustment was performed \citep{infrastructures8040066}, \citep{Kheng2005ColorSA}. Then the pixel intensities were changed again by means of histogram equalization \citep{infrastructures8040066}, \citep{SPENCER2019199} and finally redistributed by means of adaptive histogram equalization. As a result, images are obtained that have made the corrosion more visible and minimized the influence of lighting and shadows. Next the background in the images was removed so that only the \gls{roi} can be seen in the images. This was achieved as follows: first, the the background is defined manually by drawing polygons into the image. Then a binary mask was generated in which the background was white and the \gls{roi} was black (zero pixels). After subtracting the background from the input image and overlaying the result with the binary mask, the result is an image that shows only the \gls{roi}. 
For this purpose, the images are transformed from the RGB color space to the YCbCr color space \citep{articleycbcr}, since the $Y$ value is the easiest and most effective way to adjust the brightness. After the pre-processing steps and the removal of the background, the scene is considered in the Cb component, as this is the best component to see the corrosion. In the last step the classification is done by thresholding \citep{SAHOO1988233}. Finally, morphological operation like dilatation \citep{Soille2004} are applied to visualize the corrosion better and to avoid interruptions in the representation. 
As result the corroded areas with uniform illumination and without unwanted objects were successfully detected with an average of $\SI{70}{\%}$ accuracy. For images with uneven illumination and interfering objects, the detection accuracy was approximately $\SI{60}{\%}$.\\
%\red{TODO: describe one more approach with another methodology}

\subsection{Deep Learning-Based Corrosion Detection} \label{sec:optic_dl}

As described in \cref{img-based-corro-detec}, automated corrosion detection is inevitable both economically and from a practical point of view. Therefore, countless AI-based methods are also being developed.

Katsamenis et. al \citep{katsamenis2020pixellevel} deals with Deep Learning-Based Corrosion Detection. For doing so he used the following model architectures: 

\begin{itemize}
    \item \gls{fcnn} \citep{7478072}
    \item U-Net \citep{ronneberger2015u}
    \item Mask R-CNN \citep{he2018mask}
\end{itemize}

With the help of these models, semantic segmentation can be carried out, so that a pixel-precise statement can be obtained about the location and magnitude of the corrosion. After semantic segmentation, the corroded areas were very well localized. However, the boundaries of a defect were not recognized as accurately. In order to obtain highly precise results, the masks that are obtained as output from the models are further processed. The results of color segmentation are combined with the results of the semantic segmentation. Color Segmentation is a very good way of extracting the boundaries of an object. If the results of the neural networks and the color segmentation are projected onto each other, a boundary refinement can be carried out to obtain highly precise results. If the results of the neural networks and the color segmentation are projected onto each other, a boundary refinement can be carried out to obtain highly precise results.
The projection is carried out as follows: First, erosion \citep{Soille2004}  is performed on the deep masks to obtain the high confidence regions. In addition, a dilation is performed on the deep masks and then a watershed segmentation \citep{watershed} is performed to obtain the color segments. Finally, both results are projected onto each other. 

A dataset consisting of 116 images was used to train and test the models. The images were captured using various devices and have different resolutions. Furthermore, the images contained different types of corrosion. The data was labeled by engineers in accordance with the relevant standard.\\
Transfer learning was used for the FCN and Mask R-CNN models. The FCN model is based on the FCN-8s \citep{7478072}. The Mask R-CNN model is based on Inception V2 \citep{szegedy2015rethinking} and was pre-trained on the COCO dataset \citep{lin2015microsoft}. However the U-Net was designed from scratch. The structure of the Encoder is given in \Cref{fig:encoder_part_u-net}.
\begin{figure}[!ht]
  \centering
  \begin{tikzpicture}[>=stealth, node distance=0.7 cm]

    % Nodes
    \node (input) [draw, rectangle] {Input};
    \node (2conv) [draw, rectangle, below of = input] {Two consecutive convolutions, size 3x3};
    \node (pool) [draw, rectangle, below of = 2conv] {pooling};
    \node (2conv2) [draw, rectangle, below of = pool] {Two consecutive convolutions, size 3x3};
    \node (pool2) [draw, rectangle, below of = 2conv2] {pooling};
    \node (2conv3) [draw, rectangle, below of = pool2] {Two consecutive convolutions, size 3x3};
    \node (drop) [draw, rectangle, below of = 2conv3] {dropout};
    \node (pool3) [draw, rectangle, below of = drop] {pooling};

    % Arrows
    \draw[->] (input) -- (2conv);
    \draw[->] (2conv) -- (pool); 
    \draw[->] (pool) -- (2conv2);
    \draw[->] (2conv2) -- (pool2);
    \draw[->] (pool2) -- (2conv3);
    \draw[->] (2conv3) -- (drop);
    \draw[->] (drop) -- (pool3);


  \end{tikzpicture}
  \caption{Encoder of the used U-Net}
  \label{fig:encoder_part_u-net}
\end{figure}

The decoder consists of three corresponding upsampling layers.\\

The precision of the different models are given in \Cref{fig:results}.
All models achieve approximately the same accuracy. The purpose of boundary refinement is evident from the improved accuracy. \Cref{fig:F1-score results} shows the achieved F1 score of the different models. If the F1 score is taken into account as the decisive metric, then it must be noted that Mask R-CNN performs best. However, the authors state that the execution time of Mask R-CNN is significantly lower than that of the other two models. 

\begin{figure}[!h]
    \centering
    \begin{tikzpicture} [scale=0.7]
    \begin{axis}[
        ybar,                                  % Balken-Diagramm
        bar width=0.5cm,                        % Breite der Balken
        %enlargelimits=0.15,                     % Abstand zwischen Balken und Achsen
        ylabel={Precision},                    % Beschriftung der y-Achse
        symbolic x coords={FCN,Mask R-CNN,U-Net},  % Beschriftung der x-Achse
        %nodes near coords,                     % Zeige Werte über den Balken
        nodes near coords align={vertical},    % Ausrichtung der Werte
        xtick=data,                            % Zeige alle x-Ticks
        ymin=0,                                % Minimale y-Wert der Achse
        ymax=1,                                % Maximale y-Wert der Achse
    ]
    \addplot coordinates {(FCN,0.7) (Mask R-CNN,0.67) (U-Net,0.75)};
    \addplot coordinates {(FCN,0.75) (Mask R-CNN,0.71) (U-Net,0.8)};
    \legend{Before boundary refinement, After boundary refinement}
    \end{axis}
    \end{tikzpicture}
    \caption{Precision of the different models before and after boundary refinement} 
    \label{fig:results}
\end{figure}

\begin{figure}[!h]
    \centering
    \begin{tikzpicture} [scale=0.7]
    \begin{axis}[
        ybar,                                  % Balken-Diagramm
        bar width=0.5cm,                        % Breite der Balken
        %enlargelimits=0.15,                     % Abstand zwischen Balken und Achsen
        ylabel={F1 score},                    % Beschriftung der y-Achse
        symbolic x coords={FCN,Mask R-CNN,U-Net},  % Beschriftung der x-Achse
        %nodes near coords,                     % Zeige Werte über den Balken
        nodes near coords align={vertical},    % Ausrichtung der Werte
        xtick=data,                            % Zeige alle x-Ticks
        ymin=0,                                % Minimale y-Wert der Achse
        ymax=1,                                % Maximale y-Wert der Achse
    ]
    \addplot coordinates {(FCN,0.72) (Mask R-CNN,0.73) (U-Net,0.7)};
    \addplot coordinates {(FCN,0.71) (Mask R-CNN,0.73) (U-Net,0.68)};
    \legend{Before boundary refinement, After boundary refinement}
    \end{axis}
    \end{tikzpicture}
    \caption{F1 score of the different models before and after boundary refinement}
    \label{fig:F1-score results}
\end{figure}

%\red{this follows; need to adjust}
%Nash et. al \citep{Nash2022} deals with Deep Learning-Based Corrosion Detection. To begin, Nash et. al reviews several previous works that have been used for semantic segmentation to detect corrosion \citep{nash1ref} \citep{nash2ref}. 

%\red{TODO: \begin{itemize}
%    \item show the Bayesian models
%\end{itemize}}

==> sections/overview.tex <==
\section{Common Patterns in Algorithms and \gls{ml} Models} \label{sec:overview}
%============================================
%           Intro
%============================================
% Motivation: examples
So far we presented both classical and \gls{ml} based approaches separately for each inspection modality. In the course of investigation, however, there are some algorithms and/or \gls{ml} architectures which are used frequently regardless of the inspection modalities or even application fields. 
% CNN
For instance, \glspl{cnn} are ubiquitously employed for computer vision based decision making tasks in many inspection modalities including the ones that are not covered in this paper: defects and/or substance classification in \gls{ut} \citep{app13010384, 9044747} and terahertz inspection \citep{wang2021convolutional}, edge detection in X-ray \citep{xiao2021development} or semantic segmentation in thermography \citep{semantic_seg_pedrayes}, optical inspection \red{@Mohamad: could you please suggest one reference?} and X-ray tomography \citep{van2022nondestructive, hena2023deep}. 
Often integrated as a part of feature extraction, \glspl{cnn} can also be used for imaging tasks such as for reconstructing the raw terahertz measurement data \citep{jiang2022machine, helal2022signal} or enhancing the resolution of \gls{ut} \red{@Han: could you please suggest one reference?} and X-ray reconstructions \citep{jiang2022machine, helal2022signal}. 
% Classical 
This is also true for classical algorithms. Although it is called differently depending on the applications, correlation based imaging is commonly used for \gls{ut} (\gls{saft}, \gls{tfm}), radar (Synthetic Aperture Radar) as well as medicine \citep{chernyakova2014fourier}. \par%Spatial filtering, also known as beamforming, is often performed with very similar algorithms for \gls{ut}, medical ultrasound, sonar, radar and wireless communications. \par

% Why do we see the patterns?
This observation makes it evident that there are common patterns how to process the data depending on the tasks instead of inspection modalities or application fields. Such patterns appear since they tackle intrinsically the same problems and thus can be formulated in the similar, if not the same, manner to solve them numerically and/or using \glspl{nn}. 
For example, reconstructing the inner structure of a test object from \gls{ut} signals can be formulated in a very similar manner as that of reconstructing X-ray \gls{ct} data or image deblurring \citep{Schuler16Deblurr}. This is because all of these tasks aim to recover unknown quantities from the observations that are caused by these unknown quantities. %These are examples of inverse problems which, given a potentially unknown causal system, recovers the unobserved causal factor from a set of (noisy) observations that are the output of the system. 
This realization motivates us to make high level connections of the references in terms of their intrinsic natures. For this purpose, we identified four intrinsic mathematical problems we commonly encounter in \gls{ndt} applications, which are \textit{inverse problems}, \textit{forward problems}, \textit{optimal design} and \textit{pattern recognition}. \par


% Description of this section
In the following subsections, each problem is discussed with the examples to make it easier to identify the intrinsic nature of a specific engineering task. The emphasis is placed on the common patterns one can see when dealing with these tasks regardless of the applications. 
% High level connections 
%Furthermore, we also discuss how the intrinsic mathematical problems can be well associated with the high level inspection perspective we discussed in \cref{section_introduction}.
% Explanation of the table
In \cref{tab:overview}, some recommended references are provided as a summary of this section. The left most column shows the mathematical problems these references intrinsically solve. The specific \gls{ndt} related tasks are listed in the second column. The third column of the table provides the list of the sections which discuss how these problems are solved for a specific inspection modality. The fourth shows common methods to solve these tasks, and the fifth column is the list of references for the corresponding methods. The color shown in the table indicates how these tasks are associated with \gls{ndt} inspection processes we discussed in \cref{section_introduction}.
% Disclaimer 1: not exhaustive list 
Admittedly, this is by no means an exhaustive collection, yet it will give a brief overview of how one can interpret and possibly solve these tasks regardless of applications. 
% Disclaimer 2: this is only ONE possibility to make connections
Note that the conceptual connections we made here is just one possibility, and they can be described and grouped differently. \par

% Benefits
The benefits of \cref{tab:overview} are twofold.
First, acknowledging such conceptual patterns lets us understand the similarities in the tasks and try a method in other modalities or application fields. In the era of \gls{ndt} 4.0, where high level problems need to be solved by machines instead of human operators, we will increasingly encounter the problems for which no stated of the art exist. However, once the nature of the tasks is identified, such common patterns can help us determine which measure, algorithm and/or ML architecture is suitable. 
% We can see where to invest
Second, categorizing the references as shown in \cref{tab:overview} makes it clear which topics are well investigated and which are still in its infancy. This can be useful for determining the direction of future research.
% Concluding
In this context, we believe the conceptual connection we present in this work will be beneficial for the future of \gls{ndt}. 

% \subsection{Other Modalities \red{put them in the corresponding part of the next section?}}
% Similar patterns can be observed in \gls{ndt} applications not covered in depth in this work. In terahertz inspection, \glspl{cnn}-based architectures are employed in classification of substances \citep{wang2021convolutional} and in \gls{ct} \citep{hung2019terahertz}, where the lack of training data is noted as a challenge. In \citep{jiang2022machine, helal2022signal}, the usage of \gls{cnn} for general image processing tasks, \gls{rf} and \glspl{svm} for classification, and \glspl{gan} for recognition and segmentation are noted. In the case of X-ray inspection, where imaging is the main task, \gls{cnn}-based architectures such as richer convolutional feature networks for edge detection \citep{xiao2021development}, 3D \glspl{cnn} \citep{van2022nondestructive} and U-Nets \citep{hena2023deep} for the semantic segmentation of tomographic data, as well as the enhancement of low resolution images \citep{ziabari2023enabling} are widespread. 

%============================================
%           Inverse problems
%============================================
\subsection{Inverse Problems} \label{sec_inverseprob}
%----- Intro
From a set of potentially noisy observations, inverse problems aim to recover the causal factors that produced the observations.  
This formulation is beneficial since the quantities of interest often cannot be directly measured. For instance, a flaw in a test object can be represented as a change in the acoustic impedance of the test object. Yet, the acoustic impedance cannot directly be observed, instead one can measure the acoustic pressures which change according to the impedance. \par

%----- Eq and notations
For identifying the common patterns in each individual task, let us consider the causal relation described as 
\begin{equation} \label{eq_causal_rel}
    y (\ncparamy) = f ( x (\ncparamx)),
\end{equation}
where $x \in \mathcal{X}$ and $y \in \mathcal{Y}$ denote the unknown causal factor and the observation, respectively, with $\mathcal{X}$ and $\mathcal{Y}$ representing the space where they belong. The operator $f: \mathcal{X} \mapsto \mathcal{Y}$ represents a forward mapping from the causal factor $x$ to its effects $y$.
The causal factor $x$ may vary over some domains, such as time and/or space. To indicate these dependencies, $x (\ncparamx)$ denotes the values of $x$ given a set of non-causal factors $\ncparamx$. The same is also true for $y$ which, in addition to the effects from $x$, may depend on other non-causal factors $\ncparamy$. 
Note that this formulation still allows us to include stochastic factors, which are not depend on $x$ such as measurement noise, in \cref{eq_causal_rel}. 
In the following paragraphs, we will show four examples of inverse problems and how they relate to each other using the formulation \cref{eq_causal_rel}. \par

%----- Denoising + deblurring + super resolution: pattern here = the NC params/domains are the same 
% Denoising
First example is denoising, where one aims to recover the underlying clean data $x$ from the noisy observations $y$. This can be formulated with the forward operator 
\begin{equation*}
    f ( x (\ncparamx) ) = x (\ncparamx) + n (\ncparamx), 
\end{equation*}
where $n (\ncparamx)$ denotes the noise component.
% Deblurring
Distortion of the data due to echo or blur can also be described with \cref{eq_causal_rel}. By considering it as a result of convolution with the blur kernel, the distorted data $y$ can be described with the operator 
\begin{equation*}
    f ( x (\ncparamx) ) = k (\ncparamx, \sigma) \ast x (\ncparamx) + n (\ncparamx)
\end{equation*}
with $k (\ncparamx, \sigma)$ representing the blur kernel parametrized by $\sigma$. 
% Super resolution 
Increasing the resolution of the observations $y$, known as super resolution, is also an inverse problem as $y$ can be considered as the result of regularly subsampling the higher resolution data $x$. This yields the formulation of the lower resolution data $y$ as 
\begin{equation*}
    f ( x (\ncparamx) ) = \Sha ( x (\ncparamx) )  + n (\ncparamx)
\end{equation*}
with the subsampling operator $\Sha$. 
% Common patterns: the NC params/domains are the same 
Note that the observations $y$ of these three examples depend on the same non-causal factors as $x$. For instance, the values of both a clean and a noisy image vary depending on the pixel. Hence, $x$ and $y$ stem from the same domain, i.e. $\ncparamy = \ncparamx$. \par

%------ Imaging
Imaging is another example of inverse problems. %and is an important data processing step in \gls{ndt} applications. 
In the context of \gls{ndt}, $x$ is typically an unobservable physical quantity, such as the electrical conductivity for eddy-current testing or acoustic impedance for \gls{ut}. Its distribution $x (\ncparamx)$ serves as a representation of the inner structure of a test object over the domain $\ncparamx$. 
The observations $y$ are the measurable or identifiable quantities, for instance the eddy-current impedance or the acoustic pressures, which can be expressed as 
\begin{equation} \label{eq_imaging}
    y (\ncparamy) = f (x (\ncparamx)) = \Phi (x (\ncparamx); \ncparamy) + n (\ncparamy).
\end{equation}
The operator $\Phi: \mathcal{X} \times \Gamma \mapsto \mathcal{Y}$ represents the measurement process with its parameters $\ncparamy \in \Gamma$. Contrary to the aforementioned three examples, some other non-causal factors such as the locations of the sensors also influence the observations in imaging. As a result, $\ncparamy$ is generally not the same as $\ncparamx$. \par

%----- Patterns
Although their operators are slightly different, all these four tasks aim to find the inverse mapping $g: \mathcal{X} \mapsto \mathcal{Y}$ which maps the observations $y (\ncparamy)$ to the causal factor $x (\ncparamx)$.
% Difficulties
In many circumstances direct inversion of $y$ is not possible, for instance if the operator $f$ cannot be obtained analytically or the cost of inversion is prohibitively expensive. Therefore, an inverse problem often becomes a problem of how to compute the inverse mapping without (explicitly) knowing or using the forward operator $f$. 
% Approach 1: direnct inversion
There are two common approaches. One is to approximate the inverse mapping by modeling the data and minimizing its modeling error. 
% Approach 2: mapping to a representation of x
The other approach seeks to find a suitable representation of $x (\ncparamx)$, instead of explicitly recovering it. This is achieved by performing the operator $h: \mathcal{Y} \mapsto \mathcal{Z}$ which maps from $y (\ncparamy)$ to a representation of the causal factor $z (x (\ncparamx)) \in \mathcal{Z}$. An example is correlation based imaging such as beamforming and \gls{saft}, where $z (x (\ncparamx))$ is the support of $x (\ncparamx)$. \par 

%----- ML patterns
Studies have shown that incorporating \glspl{nn} can be beneficial to solve inverse problems. 
\glspl{nn} can approximate the inverse mapping in a vanilla manner \red{@Ozan: could you please suggest one/two references?} or based on the domain knowledge \citep{raissi2019physics, Karniadakis21pinnreview}, overcoming the computational limitation of numerical methods.
For speeding up the estimation procedure, \glspl{nn} can be integrated into conventional estimation methods by replacing their computationally expensive process \citep{gregor2010learning}. 
Alternatively, \glspl{nn} can be used as a post processing step to increase the estimation accuracy, when applied to the estimates obtained with the mapping $h$ \red{@Han: could you please suggest one/two references?}. \par  

%============================================
%           Forward problems
%============================================
\subsection{Forward Problems} \label{sec_forwardprob}
%----- Intro
Given a causal relation \cref{eq_causal_rel} we consider in the previous section, forward problems seek to obtain the effects $y$ from the known causal factor $x$. In the context of \gls{ndt}, the solution of a forward problem yields a synthesized version of observations described in \cref{eq_imaging}.
% Task
Though it is not directly related to the actual inspection processes, forward problems indeed play a crucial role in \gls{ndt}. For instance, forward operations are often included as a part of solving an inverse problem for modeling data as discussed in the precious section. 
For many \gls{ml} based approaches, solving a forward problem is highly beneficial, since the lack of quality data has been frequently identified as a major bottleneck regardless of their tasks \citep{cantero2022deep}. \par

%----- Eqs and notations
For most cases with \gls{ndt} applications, the forward operator $f$ includes the differential operators describing the underlying physical phenomenon, such as Maxwell's equations, wave or heat equations. As a result, its solution $y$ needs to satisfy the underlying \gls{pde}
\begin{equation} \label{eq_diffop}
    \mathcal{D} (y (\ncparamy); \pdeparam) = 0,
\end{equation}
where $\mathcal{D}$ denotes a differential operator parametrized with $\pdeparam$. 
%----- Patterns 
% difficulties 
As is the case with inverse problems, the difficulty with forward problems lies in identifying the forward operator $f$. In most cases, the forward operator $f$ cannot be obtained analytically from \cref{eq_diffop} or requires prohibitively high computation. Consequently, $f$ needs to be approximated. 

%----- Approaches
% Exact solution of PDE
A conventional approach is to solve \cref{eq_diffop} from a set of local equations using numerical solver such as finite element methods. The obtained solutions $ \hat{y} (\ncparamy)$ are guaranteed to satisfy the underlying \gls{pde}, yielding the most accurate modeling. However, its computational complexity and limited scalability may not be desirable for many circumstances. 
% Convolution with kernels
To circumvent these limitations, one can avoid exactly solving \cref{eq_diffop}. This is achieved by formulating the forward operator $f$ as a convolution
\begin{equation} \label{eq_fwkernel}
    f(x (\ncparamx); \ncparamy) = \psi (\ncparamx, \ncparamy) \ast z ( x (\ncparamx)),
\end{equation}
where $\psi$ is the kernel mimicking the measurement operator $\Phi$ in \cref{eq_imaging}, and $z ( x (\ncparamx))$ is a representation of the known causal factor. Note that $z ( x (\ncparamx))$ becomes $x (\ncparamx)$ if $z$ is an identity operator. As an example, the kernel $\psi(\ncparamx, \ncparamy)$ can be the first order Born approximation with $z (x (\ncparamx))$ being the support of $x(\ncparamx)$ \red{please correct if it is wrong}.
Since it does not exactly solve \cref{eq_diffop}, the solutions of \cref{eq_fwkernel} innately include the modeling error, making selection of the kernel a decisive factor. 

%----- ML patterns
For solving forward problems, \glspl{nn} have been demonstrated as effective tools as well. 
Numerous efforts have been paid to have \glspl{gan} learn the suitable kernel in \cref{eq_fwkernel}. With such approaches, a popular selection of the network input $ z (x (\ncparamx))$ is a binary masking operator which simplifies the inner structure of a material. 
Using \glspl{nn} as a functional approximate of the forward operator $f$ is another possibility, which can be performed in a vanilla manner using \glspl{nn} \citep{Moseley20vanilla} or by satisfying the underlying \gls{pde} \cref{eq_diffop} using \glspl{pinn} \citep{moseley2020solving, Song2021pinnhelmholtz}. 

%============================================
%           Optimal design
%============================================
\subsection{Optimal Design} \label{sec_optdesign}
Optimal design deals with the tuning of experimental parameters which can be freely chosen, and which impact the information content of measurement data with regards to parameters of interest. More broadly, the way measurement data is collected is modified so that subsequent processing and estimation tasks become simpler. Optimal design deals with problems which can be broadly formulated as follows. During an experiment, a physical phenomenon generates measurement data $\bm{y} = \bm{y}(\bm{\phi}, \bm{\theta})$, where $\bm{\phi}$ are experiment parameters that can be freely chosen (e.g. the location, number, and type of sensors employed) and $\bm{\theta}$ are parameters we are interested in. A function $f$ is applied to the measurement data $\bm{y}$ to obtain an estimate $\bm{\hat{\theta}}$, or more generally, a function $g(\bm{\theta})$ of the parameters of interest. This means $f : \bm{y}(\bm{\phi}, \bm{\theta}) \mapsto g(\bm{\theta})$ is the task to be performed with the measurement data $\bm{y}$. The performance with which the task can be performed depends on the experiment parameters $\bm{\phi}$, as these parameters affect the measurement data. This performance can be measured through the judicious choice of a function $h : g(\bm{\theta}) \mapsto p$, where $p \in \real$. Optimal design then refers to problems of the general form
\begin{align}
    \max_{\bm{\phi}} h(f(y( \bm{\phi}, \bm{\theta} ))).
\end{align}
Such problems benefit greatly from \gls{ai} due to several factors. First, when accurate physical models for the measurement data are involved, closed form expressions or approximations for $\bm{y}(\bm{\phi}, \bm{\theta})$ may be unavailable, as is the case with differential equations and \glspl{pinn} \red{[could cite some PINN papers here]}. Even when a closed form expression is available, the model $\bm{y}$ may be discontinuous in $\bm{\phi}$, resulting in difficult optimization tasks that do not directly admit gradient-based methods. An example of this is the case of optimal sensor placement and sparse array design in the discrete case, which take the form of combinatorial problems and involve the sampling of discrete random variables \red{[we can cite han's papers here]}. The performance measure $h$ may suffer from similar limitations as well \red{[consider citing the papers on sparse rate reduction that emre and i posted on discord, or mention the spark of a matrix as a possible performance constraint]}. One or more of these components can be substituted by neural networks that approximate the desired behavior.

%============================================
% Pattern recognition
%============================================
\subsection{Pattern Recognition}
%----- intro
Pattern recognition can be found ubiquitously in many data analysis and decision making tasks. 
%----- Eqs and notation
In general, given the input space $\mathcal{X}$ and the desired output space $\mathcal{Y}$, we only have an access to their samples $x \in X \subset \mathcal{X}$ and $y \in Y \subset \mathcal{Y}$. The goal of pattern recognition is to estimate the true mapping $g: \mathcal{X} \mapsto \mathcal{Y}$ from the available, often limited number of, samples. This is formulated as a problem of finding the mapping $\hat{g}: X \mapsto Y$ as closely as possible to the true mapping $g$. 
% Eq & notation
Mathematically, a pattern recognition task can be described as two consecutive mappings
\begin{equation} \label{eq_patrec}
    y (\ncparamy) = g (x(\ncparamx) ; \bmomega_{g}) = h (f( x(\ncparamx) ; \bmomega_{f}); \bmomega_{h}).
\end{equation}
% Non-causal factors/domains
Here, we follow the same notation as in \cref{sec_inverseprob} to show the dependency of the input and the output on other factors as $x (\ncparamx) \in \mathcal{X}$ and $y (\ncparamy) \in \mathcal{Y}$.
The operator $f: \mathcal{X} \mapsto \mathcal{Z}$ maps the input data $x \in \mathcal{X}$ to its function $z = f ( x(\ncparamx) ; \bmomega_{f}) \in \mathcal{Z}$, which is followed by another mapping $h: \mathcal{Z} \mapsto \mathcal{Y}$. The mappings $g$, $h$ and $f$ are parametrized by $\bmomega_{g}$, $\bmomega_{h}$ and $\bmomega_{f}$, respectively. 
% Two cases
There are two cases in pattern recognition based on the outputs  $y(\gamma) \in Y$: when the outputs are known and when they are not. 

% Case 1: when the outputs are known
If the outputs are known and directly attainable, the mapping $g$ can be inferred statistically based on the available samples. This is achieved by implicitly maximizing the conditional distribution $P (y \vert x)$ of the training data set. This type of pattern recognition is often performed for a decision making purpose.
% Example tasks
One of its examples is classification. Using \cref{eq_patrec}, the mapping $f$ can be considered as a data processing step and yields $z (\ncparamx; \ncparamy)$ as the post-processed version of $x(\ncparamx)$. The output $y = y(\ncparamy)$ is a single label of the input $x(\ncparamx)$. 
%
By repeating classification tasks, some objects and/or occurrences in the input data can be localized. Such localization tasks are often computed block-wise to reduce the search area, which can be expressed with $z(\ncparamx ; \ncparamy)$ as the block of the input data and $\ncparamy$ representing the size and the location of the block. 
For a block $z(\ncparamx ; \ncparamy) $, the mapping $h$ returns either a single label (detection) or multiple labels with the same size as that of the block to specify the exact boundaries (segmentation). 
% Difficulties
Since the mapping $g$ is estimated based on the sample statistics, the quality of the samples is the decisive factor when performing these tasks. Augmenting and synthesizing the input data can be helpful to overcome this limitation. A caution needs to be taken with data processing procedure, such as feature extraction, as it may enhance or lose the descriptive patterns in the raw data. \par

%---- Case 2: when output y is unknown = feature extraction
Indeed, feature extraction can also be considered as a pattern recognition task, where the outputs are typically not explicitly known. This is equivalent to find the mapping $f$ of \cref{eq_patrec} in an unsupervised manner. 
% Difficulty + Approaches (difficulty = outputs are unknown)
Since the true outputs are generally unknown, some optimality criteria should be set to find a suitable mapping $\hat{f}$. 
% Approach 1: based on some beliefs about the data 
One approach is to choose $\hat{f}$ so that it satisfies some beliefs about the data such as domain knowledge or statistical assumptions. Examples of this type include simple filtering (using the knowledge of the relevant frequency range of the signals), \gls{pca} (assuming the orthogonality of the relevant components), independent component analysis (assuming that the relevant components are statistically independent and have non-Gaussian distribution) and $k$-means clustering (assumption of intra-class spherical distribution and homoscedasticity).
% Difficulty + pattern
Note that this type of feature extraction does not aim to improve the accuracy of the successive decision making task $h$. 
For this reason, it is also called as \textit{unsupervised} feature extraction and often used for exploratory purpose.
% Approach 2: end-to-end = based on the performance of the successive task
Another approach is to learn the features from the available samples, such that the resulting features positively affect the performance of the successive task $h$. 
This includes \gls{lda} \citep{Sarg19dg, Cy21}, \gls{svm} \citep{Calderbank2009CompressedL} and \gls{ml} based end-to-end methods where features are extracted in the intermediate steps prior to decision making. 
% Difficulties + problems
Since the learning is based on the available samples, the quality of the samples determines the performance. 


%============================================
% Table
\centering
\begin{table*}
    \scalebox{1.0}{\input{tikz_tables/table_overview.tex}}
    \caption{
        Summary of the methods used for common \gls{ndt} tasks. %
        References are categorized according to the intrinsic mathematical problem they are dealing with as discussed in \cref{sec:overview}. %
        Each color in the table is associated to a \gls{ndt} inspection process: green for data enhancement, pink for data synthesization, orange for measurement operation and blue for decision making. 
        Note that end-to-end end-to-end \gls{ml} methods often perform feature extraction implicitly. These methods are not shown as feature extraction, instead categorized into their targeted decision making tasks. 
    }
    \label{tab:overview}
\end{table*}


==> sections/pinn.tex <==
\section{Physics-aware Data Synthesization} \label{sec:pinn}

Since data acquisition is often very time consuming for \gls{ndt} applications, preparing sufficient amount of well labeled data is typically very challenging. Synthesizing high quality data is hence beneficial especially for AI based approaches and has been gaining interests \red{To-Do: add some references}. %
Contrary to the vanilla NNs, PINNs are attractive for synthesizing data as they are designed to obey the underlying physics. \red{To-Do: add more benefits of PINN data synthesization: effective training using only small data sets, mesh-free, the same network can be used for both forward and inverse problens, PINNs work well with very complicated geometries and/or in very high dimensions that are not feasible for conventional numerical solvers such as finite element method} \citep{raissi2019physics}. \par

In PINN configurations, a successfully trained network is a direct functional approximation of the partial differential equation (PDE) of interest. 
PINNs can be considered as the learning approaches which embed the underlying physics as learning bias \citep{Karniadakis21pinnreview}.
This is achieved by including the given boundary conditions and the underlying PDE as constraints into the loss function of the network \citep{raissi2019physics}. Generally, the loss function is the weighted sum of the unsupervised PDE loss (physics loss) and the supervised data loss of the initial and boundary conditions (boundary loss) as discussed in Section \ref{section_tomography}. While the physics loss reinforces the network to satisfy the underlying physics, the boundary loss ensures that the network learns a unique solution \citep{moseley2020solving}. \par

% Boundary conditions
In general, the difficulty of configuring PINNs lies in selecting the weights for the joint loss function, i.e. for the physics loss and the boundary loss. \red{To-Do: what happens when the weights are not carefully selected} \par

% Activation functions 
Furthermore, it has been reported that a selection of the activation function effects the performance of PINNs \citep{Cheng2022pinnsinusoid}. \red{To-Do: more explanation on how they affect the performance}.

% Variational PDEs
Variational forms are another approach to solve PDEs. \red{To-Do: more explnataion on variational forms} Based on the principle of the least action, variational forms solve second order differential equations as stationary points of the underlying action functional \citep{Offen2023pinnvariational}. In this way, instead of directly solving the second order PDEs, variational forms only need to deal with the first order derivatives. \red{To-Do: add more benefits of variational forms, especially why it is good to have only first derivatives}

% Overview
In this section, we present PINNs approaches for data synthesization, i.e. forward problems. An effective use of PINNs for the wave equation is firstly demonstrated in \citep{moseley2020solving}, presenting remarkable results for approximating 2D wave equations with absorbing boundary. \red{To-Do: more comments on other papers}.
We first discuss how the weights can be selected for the joint loss function specifically for the wave equations. We then review how activation functions can affect the performance of PINNs and what we can do about them \red{To-Do: elaborate here}. Lastly, we briefly review variational approaches, which showcase promising results for solving the wave equations as well. \par



Studies to consider are...
\begin{itemize}
    \item dynamic PDEs (no steady state ones)
    \item mesh-free approach (continuous space), how about time..?
    \item inhomogeneous PDE (= with source)?
\end{itemize}

%\clearpage

% Summary table (alphabetical order)
\rotatebox{90}{
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
    \hline
    % Header
    &&&&&&&&&\\
    Reference & Year & Application & Differential eq. & Domain & 
    Network & Activation & BC/IC handling & Boundary & Medium \\
    &&&&&&&&&\\
    \hline
    % Moseley
     Mosely \textit{et al}& 2020 & seismology & inhomogeneous & time & 
     dense & softplus & curriculum & absorbing & isotropic \\
     \citep{moseley2020solving} & & & 2D wave & & 
     & & learning & & Marmousi\\
     \hline
     % Song Helmholtz
     Song \textit{et al}& 2021 & seismology & inhomogeneous & freq. & 
     dense & adaptive & PML & absorbing & anisotropic \\
     \citep{Song2021pinnhelmholtz} & & & 2D wave & &
     & sine & model & & Marmousi \\
     \hline
     % Yang: PINN with GANs
     Yang \textit{et al}& 2020 & \red{sensor} & SDE & freq. & 
     GANs & tanh & & absorbing & homogeneous, \\
     \citep{Yang2020pinngans} & & \red{networks?} & (1D diffusion) & 
     & & & & & noisy\\
     \hline
\end{tabular}
}

==> sections/terahertz.tex <==
\section{Terahertz} \label{section_terahertz}
\red{WIP: only gathering references for now, but the feel is overall similar to ultrasound}
\begin{itemize}
    \item \citep{wang2021convolutional} usage of thz and CNNs to detect and classify liquids (liquid contraband :P)
    \item \citep{hung2019terahertz} very short paper on the usage of CNNs for terahertz tomography. not sure whether to include this one yet
    \item \citep{jiang2022machine} review paper on the usage of ML with terahertz imaging, spectroscopy, etc.
    \item \citep{helal2022signal} IEEE sigproc magazine article reviewing general terahertz techniques and machine learning
\end{itemize}

==> sections/tomography.tex <==
\subsection{{Computed Tomography and Full Waveform Inversion}} \label{section_tomography}

\han{(16 references in 3.2)}

In \gls{uct}, cross-sections of the internal structure of an object are created based on a model of the ultrasound propagation process and measurements collected from sensors placed on the object's surface \citep{khairi2019ultrasound}. The cross-sections are quantitative in nature, accurately describing the physical parameters of the object under test. Traditional \gls{uct} methods rely on the first-order Born approximation \citep{gubernatis1977born} and straight ray models. This results in computationally efficient algorithms similar to those employed in X-ray imaging. An example of this is presented in \citep{zielinska2018non}, where the \gls{art}, which is commonly employed in X-ray imaging, is used to produce slowness maps of masonry pillars based on through-transmission measurements. These slowness maps are later used to compute the Young's modulus. The authors of \citep{haach2016qualitative} focus directly on the slowness map, which they obtain by applying the \gls{sirt} on through-transmission data. However, these models ignore phenomena such as refraction and multiple scattering, which in turn limits resolution and quantitative interpretability \citep{duric2007detection}. 

In recent years, the approach commonly employed in geophysics and seismology has increasingly drawn the attention of the ultrasound community. Dubbed \gls{fwi}, this approach focuses on solving \cref{eq_wave,eq_helm} accurately to simulate a more realistic propagation process \citep{virieux2017introduction}. This is generally formulated as a nonlinear least squares problem of the form
\begin{align} \label{eq_fwi}
    \min_{\bm{\gamma}} \left\Vert G(\bm{\gamma}) - \bm{p}_{\mathrm{rec}} \right\Vert_2^2
\end{align}
where $G$ is a nonlinear function mapping the parameters of interest $\bm{\gamma}$ to simulated measurement data; traditionally, a differential equation solver. We note in passing that the problem can be alternatively formulated in the frequency domain by using $\tilde{\bm{p}}_{\mathrm{rec}}$ instead.

\gls{fwi} has successfully been applied to challenging scenarios in medical ultrasound, e.g. for high-resolution imaging of the brain \citep{guasch2020full}. However, \gls{fwi} remains a challenging task: the computational effort involved in accurately and repeatedly simulating ultrasound propagation requires proper infrastructure. Additionally, the problem in \cref{eq_fwi} is ill-posed and requires proper regularization. 

Neural networks offer assistance in tomography with and without \gls{fwi}. Instead of addressing forward modeling and inversion with standard techniques, deep learning can substitute components in the process, or replace it in its entirety. In \citep{klosowski2020maintenance} the authors wish to detect inclusions, as well as their shape and size, inside reactor tanks. The parameter $\bm{\gamma}$ is taken as a binary mask denoting the presence of inclusions. Training data is generated synthetically, and a preprocessing step $f: \bm{p}_{\mathrm{rec}} \mapsto \bm{\tau}$ maps the measurement data $\bm{p}_{\mathrm{rec}}$ to a vector $\bm{\tau}$ containing the first time of arrival per channel. Next, a classification \gls{cnn} $\Psi$ performs the mapping $\Psi: \bm{\tau} \mapsto \hat{\bm{\gamma}}$. To do so, the authors generate synthetic binary defect maps $\bm{\gamma}_{\mathrm{synth}}$ and consider a cost based on the difference $(\Psi(\bm{\tau}) - \bm{\gamma}_{\mathrm{synth}})$. In \citep{lahivaara2018deep}, forward modeling is done using a variant of the Galerkin method to compute $G: \bm{\gamma} \mapsto \bm{p}_{\mathrm{rec}}$, while inversion is carried out using a \gls{cnn} $\Psi: {\bm{p}}_{\mathrm{rec}} \mapsto \hat{\bm{\gamma}}$. The parameter $\bm{\gamma}$ in \citep{lahivaara2018deep} represents the material parameters, such as porosity, of test objects immersed in a water tank. Like in \citep{klosowski2020maintenance}, the authors of \citep{lahivaara2018deep} take a task-based approach instead of using \cref{eq_fwi}. The cost function then takes the form $\Vert \Psi(\bm{p}_{\mathrm{rec}}) - \bm{\gamma} \Vert_2^2$, where training takes place based on a set of reference parameters $\bm{\gamma}$. Other examples of \gls{uct} in the \gls{ndt} context are reviewed in \citep{cantero2022deep}, where the overall trend shows \glspl{cnn} emerging as powerful tools in computed tomography.

Although \gls{uct} is found comparatively more often in medical applications than in \gls{ndt}, it is still in its infancy in medical imaging. Nevertheless, medical imaging has seen more progress in the integration of \gls{uct} and artificial intelligence. A standout example of this can be found in \citep{long2023deep}, where the authors are interested in reconstructing the speed of sound maps $\bm{\gamma}$ using only a small number of sensors. In contrast with the aforementioned papers, a network is employed directly in the image domain. A low-resolution image $\bm{\bar \gamma}$ is obtained by first solving a nonlinear optimization problem involving a bent ray model and, similarly to \citep{klosowski2020maintenance}, the first arrival time per channel. Next, a U-Net \citep{ronneberger2015u} performs the mapping $\Psi: \bm{\bar \gamma} \mapsto \hat{\bm{\gamma}}$. This U-Net is trained so that the resulting speed of sound maps is as similar as possible to reference maps obtained with a larger number of sensors. That is to say, given a reference high-resolution speed of sound map $\bm{\gamma}$, the U-Net is trained based on the reconstruction fidelity $\Vert \Psi(\bm{\bar\gamma}) - \bm{\gamma} \Vert_2^2$. Implementations similar to the aforementioned \gls{ndt} ones also exist. As an example, in \citep{feigin2019deep}, a speed of sound map $\bm{\gamma}$ is computed from a small number of plane wave insonifications by using \glspl{cnn}. Data is simulated using Matlab's k-wave toolboox to compute $G: \bm{\gamma} \mapsto {\bm{p}}_{\text{rec}}$, while the \gls{cnn} performs the inversion ${\bm{p}}_\mathrm{rec} \mapsto \hat{\bm{\gamma}}$. The prevalence of \glspl{cnn} is medical imaging applications is also notable.

A separate approach to modeling and inversion is provided by \glspl{pinn} \citep{raissi2019physics, moseley2020solving, rasht2022physics}. \glspl{pinn} breaks away from the previous patterns of using classical methods of forward modeling. Instead, the focus is shifted onto the representation of solutions to the governing differential equations. To this end, a neural network $u_{\bm{\theta}}: (\omega, \bm{x}) \mapsto {p}(\omega, \bm{x})$ with internal parameters $\bm{\theta}$ is employed, noting that a similar formulation is possible in the frequency domain. 

The power of this approach comes from using a simple neural network, usually a shallow \gls{dn} that does not explicitly depend on $\gamma$, and enforcing desirable properties on it through the judicious choice of a cost function. The cost should incorporate the governing equations and all available initial and boundary conditions. As an example in the frequency domain, consider the Helmholtz equation. Based on \cref{eq_helm}, a term of the form
\begin{align} \label{eq_pinn}
    \left\Vert (\nabla^2 + k^2)(\tilde u_{\bm{\theta}}) + \tilde{s} \right\Vert^2
\end{align}
can be included in the cost function. The minimization of this term directly promotes the property that $\tilde u_{\bm{\theta}}$ should be a feasible solution to the Helmholtz equation. Importantly, \cref{eq_pinn} is written in its continuous form to highlight that $\tilde u_{\bm{\theta}}$ is a function that solves the differential equation and can be evaluated anywhere in the computational domain $(\omega, \bm{x})$, for any frequency and spatial position. In practice, a set of points from the computational domain of interest should be chosen, yielding a sum over the chosen points. This term would be added as a regularizer to a conventional data fidelity term of the form $\Vert \tilde u_{\bm{\theta}}(\omega, \bm{x}) - \tilde{p}_{\text{rec}}(\omega, \bm{x}) \Vert^2$. Similar terms can be formulated for the initial and boundary conditions, or these can be learned implicitly if enough data is available.

In the case of inverse problems, the parameter $\gamma = k$ can be replaced with a neural network $\Psi_{\bm{\phi}}: (\omega, \bm{x}) \mapsto k(\omega, \bm{x})$ with internal parameters $\bm{\phi}$. After an initial training stage for $\tilde u_{\bm{\theta}}$ with data from a known reference medium, one can then train $\tilde u_{\bm{\theta}}$ and $\Psi_{\bm{\phi}}$ simultaneously from measurement data of the object of interest by considering the problem
\begin{align} \label{eq_pinn_inv}
    \argmin_{\bm{\theta}, \bm{\phi}} \left\Vert (\nabla^2 + \Psi_{\bm{\phi}}^2)(\tilde u_{\bm{\theta}}) + \tilde{s} \right\Vert^2 + \lambda \left\Vert \tilde u_{\bm{\theta}} - \tilde{p} \right\Vert^2 
\end{align}
with possible additional terms accounting for boundary and initial conditions. An example of this approach can be found in \citep{shukla2020physics}, where \glspl{pinn} are employed in the estimation of the speed of sound maps to locate cracks with high accuracy based on time domain data.

The tomography and \gls{fwi} approaches discussed in this section can roughly be categorized as shown in \cref{tab:tomo}.

\begin{table}[H]
\caption{Classification of \gls{ml}-aided \gls{uct} and \gls{fwi} approaches \red{(if anyone can help me come up with better names for the approaches, that'd be great)}}
\label{tab:tomo}
\begin{center}
\begin{tabular}{ m{1.8cm} m{2.6cm} m{2.6cm} } 
 \hline
    Approach & Forward method & Inverse method\\
 \hline
 \hline
    Direct & classical & CNN   \\
    Two-step & classical & preprocessing + CNN \\
    PINN & DN & DN \\
 \hline

\end{tabular}
\end{center}
\end{table}

==> sections/us_classification.tex <==
\subsection{Ultrasound Data Classification} \label{sec:ut_classification}

\han{(28 references in 3.3, could consider reducing when necessary)}

In the era of \gls{ndt} 4.0, the integration of \gls{dl} and \gls{ml} methods in ultrasound defect classification techniques changed the overall performance and efficiency of the industrial implementations significantly. Each year, smarter, more robust, higher accuracy, and cost-effective algorithms are being developed. Various classification methods have been applied in \gls{ut}, with their success largely depending on the availability and quality of the training data \citep{SUN2023106854}. Although data acquisition is a critical initial step in ultrasound-based classification frameworks, it will not be mentioned in this section. Considering reliable measurement data is available at hand, the focus of this section is to give a comprehensive review of the recent developments in ultrasound classification in \gls{nde} by giving prominent examples of the papers using a classification workflow that combines feature extraction and classification techniques. Extracting the features of the measured signal is a crucial work, especially in the context of ultrasound, where the sound data can be represented in myriad different ways. The feature extraction step quantifies and identifies the key characteristics of the data, enabling the classification algorithms afterward to efficiently distinguish between the various classes with high accuracy. Combining signal processing methods, including time-frequency-scale representations of the signal and dimensionality reduction algorithms, with \gls{dl} networks and \gls{ml} classifiers proved to be effective as shown in the examples below.

Due to their ability to provide both time and frequency domain information of the signal simultaneously, the \gls{stft} and wavelet transform \citep{57199} have been used in ultrasound classification for extracting strongly informative features. While STFT can be considered as a traditional technique, there are still recent usages in NDE subsectors, such as structural health monitoring for railway tracks, by employing CNNs after the feature extraction \citep{app13010384}. Regarding the identification of rail defects, the wavelet transform is also proved to be a valuable tool for feature extraction. In \citep{JIANG2019455}, wavelet coefficients, energy, and local entropy are utilized for extraction of the representative features of the data alongside \gls{kpca} for the dimensionality reduction algorithm. The authors of \citep{JIANG2019455} propose utilizing \gls{svm} in the classification task. In \citep{LV2023102752}, three  \gls{ml} classification techniques, in particular adaptive boosting, \gls{xgboost} and \gls{svm}, are compared all by accompanying wavelet energy features for classifying the defects with laser ultrasound signals.

Addressing another crucial \gls{nde} subsector, in \citep{9044747}, \gls{dwt} is applied in a pipeline weld inspection using \gls{emat}. The high-level features from the time-frequency representation of A-Scan signals are used to classify the welding defects in a gas pipeline. The wavelet features are then given into a \gls{cnn}-\gls{svm} classifier. Different solutions to the problem of classifying ultrasound signals in welding applications are proposed in a similar manner as employing the wavelet coefficients-based extracted features in \citep{Chen2023} with \gls{abc}-\gls{svm} and in \citep{pawarpranav} with \gls{cnn}. Another efficient implementation of combining the extracted wavelet coefficients and \glspl{cnn} is presented in \citep{electronics10151772} and \citep{arbaoui2021} for identifying and monitoring the cracks in concrete, respectively.

In fact, the wavelet decomposition is quite powerful that its effect on classification accuracy is demonstrated in \citep{Sudheera2020} by comparing two methods, one using \gls{lstm} directly on the ultrasonic signals, and the other one applying \gls{lstm} after the wavelet feature extraction carried out. Yet another strength of the wavelet transform is extracting definitive features so that they can be used with unsupervised machine learning algorithms such as Gaussian Mixture Modeling, Mean Shift Clustering, and K-means Clustering \citep{8926078}.

Furthermore, apart from taking the wavelet coefficient-based values directly as features, the usage of wavelets in reliable feature extraction can be utilized as the preprocessing step as well. In \citep{OLIVEIRA2020106166}, wavelet transform is carried out to denoise the data so that the features represent the signal more efficiently compared to the noise in the context of detecting the possible damages in wind turbine blades.

There exist different adaptations of the wavelet-based features, such as the \gls{ewt} \citep{6522142}, which decomposes the signal into a finite number of components adaptively without necessitating prior knowledge of the time-frequency information of the signal. In \citep{Jayasudha2022}, it is demonstrated that \gls{ewt} as a feature extraction algorithm can be combined with Deep Convolution Neural Network to classify the phased array ultrasonic test signal. Additionally, \gls{ewt} is originally inspired by another feature extraction method called \gls{emd} \citep{huang1998empirical}, which is utilized to empirically break down data into its intrinsic oscillatory modes that include the local time-scale information of the signal. An implementation of \gls{emd} alongside \gls{dwt} and various significant features, including entropy and crest factor, is shown in \citep{zhang2021classification} for classifying the damage and fracture process in wood by using acoustic emission signals. After acquiring the features, an \gls{lda} classifier is carried out. Whereas mentioning the decomposition of the ultrasound signals into components, \gls{vmd} \citep{vmd} stands out with a predefined mathematical framework by solving a constrained variational problem in a non-recursive manner. Apart from those key differences from \gls{emd}, \gls{vmd} is also used in the classification of ultrasonic measurements as in \citep{wood} for wood hole-damage classification, and in \citep{9247428} for denoising the signal before obtaining the final extracted features.

Other than the standard non-sparse datasets, ultrasound signals can also be represented sparsely by exploiting the spatial sparsity of measurement area and the appropriate dictionary matrix as in \citep{schiffner2019random}. As an initial example of the sparse data classification with low-quality reconstruction data, the authors in \citep{lohit2016direct} replace the iterative sparsity-promoting algorithm with \gls{cnn} after transforming the data in measurement domain to the image domain by applying simple projection as ${\boldsymbol{\bar{\gamma}}} = \bm{G}\herm\bm{p}_{\mathrm{rec}}$. Afterward, the less accurate data ${\boldsymbol{\bar{\gamma}}}$ is given as input of \gls{cnn}, which is constructed using different architectures like LeNet-5 model \citep{726791} and CaffeNet \citep{jia2014caffe} depending on the types of data. The accuracy rate in the testing phase is compared with another sparse signal classification algorithm called Smashed Filters \citep{davenport2007smashed}, which creates distinct parametric manifolds using the \gls{mle} to find the parameters of those different manifolds and then classify the data among those estimated manifolds. The performance results show that the accuracy of the \gls{cnn}-based classification of the compressed measurements outperforms the Smashed Filters implementation. 

Deviating from extracting information from data with the signal processing techniques to only data-driven methods, in \citep{8863361}, a \gls{fcnn} and a \gls{gru} are applied to the signal to extract the features, and a softmax layer is carried out afterward for the classification task. Moreover, in \citep{HA2022106637}, an autoencoder structure is utilized to understand the defect-free signal characteristics and detect the anomalies in the signal when there is a defect. In the cases that ultrasound data can be represented sparsely, the paper \citep{Calderbank2009CompressedL}, which classifies the data directly in the measurement domain, can be investigated. This paper shows that soft-margin SVMs classifying the data in the compressed measurement domain provide as accurate results as the best possible classifier in the original data domain. In other words, reconstruction of the original data is not necessary in the classification task using soft-margin SVMs which reduces the computational complexity considerably, especially if the original data size is much bigger than in the measurement domain.

Last but not least, a comprehensive analysis of the recent enhancements in \gls{nde} with ultrasound data using numerous \gls{dl} techniques utilized as feature extraction methods, such as autoencoders, \glspl{gru}, \glspl{rnn}, \glspl{cnn} is discussed in \citep{CANTEROCHINCHILLA2022102703}.

==> shrink_ultrasound/ultrasound.tex <==
\section{Ultrasound} \label{section_ultrasound}
Ultrasound signals, \han{characterized by frequencies from 20 kHz to the gigahertz range and beyond human hearing\cy{and beyond human hearing - could be left out}, are pivotal in computational imaging, especially in \gls{ndt}. A key technique in this domain} is pulse-echo ultrasound imaging, \han{which} involves the capture and utilization of scattered echoes arising from inherent inhomogeneities within the measurement area.

In its simplest form, ultrasound data can be modeled via the wave equation \citep{verweij2014simulation}, so that the measured pressure field $p$ obeys
\begin{align} \label{eq_wave}
    \nabla^2 p - \frac{1}{c^2} \frac{\partial^2 p}{\partial t^2} = -s.
\end{align}
In \eqref{eq_wave}, $p = p(t, \bm{x})$ is a pressure field that depends on the time $t$ and position $\bm{x} \in \real^d$ for a $d$-dimensional space. The speed of sound $c = c(\bm{x})$ may in general vary over space due to changes in density and compressibility, and the term $s = s(t, \bm{x})$ represents sources in the medium. Alternatively, when working with a monochromatic field or after separation of variables, the frequency domain representation of the field obeys the Helmholtz equation, meaning
\begin{align} \label{eq_helm}
    \nabla^2 \tilde p + k^2 \tilde p = -\tilde s,
\end{align}
where quantities with a tilde $\tilde{(\cdot)}$ are frequency domain counterparts to the corresponding quantities without the hat.cy{sorry, what is meant by hat?} As a result, $\tilde p = \tilde p(\omega, \bm{x})$ and $\tilde s = \tilde s(\omega, \bm{x})$ depend on the angular frequency $\omega$, and all quantities including the wavenumber $k = k(\omega, \bm{x})$ can vary over space.

A common practice is to obtain approximate solutions to \cref{eq_wave,eq_helm} by discretizing them into systems of linear equations. In the time domain, the problem can be formulated as
\begin{align}
    \bm{p} = \bm{G \gamma},    
\end{align}
where $\bm{p}$ is obtained by discretizing $p$, e.g. along the temporal and spatial axes. The matrix $\bm{G}$ is referred to as the \emph{model} or \emph{measurement} matrix, and its formulation depends on the task. Similarly, the vector $\bm{\gamma}$ encodes the sought-after parameters, and its exact definition depends on the application.

Many ultrasound-based \gls{ndt} techniques cy{for someone who has not much knowledge of US, whicht different techniques are ment?} revolve around estimating the speed of sound $c$, the wavenumber $k$, or the underlying physical parameters that determine them. Quantitative and qualitative estimates of these parameters are employed in detection, localization, imaging, classification, and more. Additionally, the amount of information about these parameters depends on the data measurement modality \cy{is this another word for DoE or experimental setup?}. As a result, the optimization of measurement parameters is another well-researched task. We discuss recent trends and open opportunities in the application of artificial intelligence to ultrasound \gls{ndt} tasks next.

\subsection{Ultrasound Imaging} \label{sec:us_ssr}

%\red{Let's rename this to ``Ultrasound Imaging'' and make it more general. We can rework equation (5) to instead show a regularized inverse problem. We can then mention sparse recovery/compressed sensing as a particular example. We'll then put the imaging sections as subsections of this one.}

Conventional techniques like \gls{pwi} and \gls{fmc} transmit several incident waves from different angles and/or locations and collect the scattered echoes in the receiver \citep{le2016plane}. These traditional techniques mostly depend on augmenting the number of transmitted signals to enhance the accuracy and resolution of the reconstruction or classification.  

A mathematical model for the received signal in the ultrasound imaging can be defined in the form of matrix-vector multiplication as
\begin{align}
{\bm {\tilde p}}_{\mathrm{rec}}={\bm G}{\boldsymbol{\gamma}} + {\bm{\tilde \eta}}.
\end{align}
where ${\bm {\tilde p}}_{\mathrm{rec}}$ is the received or measured frequency domain signal vector carrying distinct samples, ${\boldsymbol{\gamma}}$ is the parameter of interest, and ${\bm{\tilde \eta}}$ represents complex additive noise. A common choice for the construction of ${\bm G}$ \cy{G is the model matrix here, too? maybe write someting like construction of model matrix ${\bm G}$} is to employ the first-order Born approximation and Green's function for a homogeneous, isotropic medium, as shown in \citep{schiffner2019random}. Following this model, the inverse scattering problem in which $\bm{\gamma}$ is estimated from the measurement data ${\bm{\tilde p}}_{\mathrm{rec}}$ can be reformulated into an optimization problem
\begin{align} \label{inverse}
\begin{array}{l l l}{{{\hat{\bm{\gamma}}}={\underset{{\boldsymbol{\gamma}}\in{\mathbb{C}^{{N_{\mathrm{el}}} \times 1}}}{\operatorname{min}}}}}&{{\|{\bm {\tilde p}_{\mathrm{rec}}}-{\bm{G}}{\boldsymbol{\gamma}}\|_{2}\leq\eta}},\end{array}
\end{align}
where $ \|{\bm{\tilde \eta}}\|_{2}\leq{\eta}$. 

One example for the solution of \cref{inverse} is the case where $\bm{\tilde p}_{\text{rec}}$ is represented sparsely by ${\bm{G}}$. In that case, it can be estimated by harnessing a reduced quantity of transmitted data without reducing performance; in some cases, even by exploiting just a single transmission \cy{and receive by the same transducer?} from each element of the ultrasound transducer array\citep{schiffner2019random, camsap23}. There are several conventional sparse data recovery algorithms, i.e. the \gls{ista} \citep{daubechies2004iterative} based on proximal gradient descent, its accelerated version \gls{fista} \citep{4959678} and the \gls{admm} \citep{boyd2011distributed} which splits the problem into simpler subproblems which separately focus on addressing the reconstruction fidelity and promoting sparsity through a penalty function. However, all of these algorithms work iteratively and come with a significant computational cost and slowness. Hence, novel methodologies based on neural networks have emerged that lower the reconstruction time without compromising the reconstruction accuracy. 

In the next sections, we explore different artificial intelligence approaches to the inverse problems involved in imaging. One approach focuses on designing conventional neural network architectures to tackle the inverse problem, while the other involves reconstruction based on the model of the data and well-known classical optimization algorithms. 

\subsubsection{Ultrasound Imaging with Conventional Deep Learning Architectures} \label{sec:ut_imaging_vanillaDL}

%\red{Rename to something like ``Ultrasound Imaging with General Architectures''. My understanding in the paragraph right below this one is that sparse recovery is anyway not exploited, but instead it's replaced by general neural networks. We can remove the emphasis from CS/sparse recovery. The first paragraph can be made a little clearer, too.}

A self-supervised auto-encoder network \han{that minimizes} the \gls{mse} between $\bm{{p}}_{\mathrm{rec}}$ and $\hat{\bm{p}}_{\mathrm{rec}}$ is employed in \citep{zhang2020self}. \han{This network processes projection of measurement data in the image domain}, i.e. the intermediate quantity ${\boldsymbol{\bar{\gamma}}} = \bm{G}\herm \bm{p}_{\mathrm{rec}}$, \han{which resembles} \gls{saft}. After the autoencoder network gives the reconstruction data $\bm{\hat{\gamma}}$ as training output, its projection to the measurement domain is calculated this time as ${\bm{\hat{p}}}_{\mathrm{rec}} = \bm{G}{\boldsymbol{\hat{\gamma}}}$. The results show that the autoencoder gives a similar \gls{cnr}, the same axial \gls{fwhm} with the conventional \gls{das} beamforming using 75 \glspl{pw} and lower \gls{fwhm} in lateral direction although it exploits only one \gls{pw}. \han{Similarly}, \sout{an algorithm} based on \gls{drl} \citep{he2016deep}, a method \sout{developed} for removing the vanishing gradient problems in the neural networks is proposed in \citep{yao2019dr2}. \han{Firstly}, the measured signal is linearly mapped to the image domain using a fully connected network as ${\boldsymbol{\bar{\gamma}}} = \bm{W}\bm{p}_{\mathrm{rec}}$ and the elements of the matrix $\bm{W}$ are learned using the conventional \gls{sgd} training algorithm. After obtaining the initial estimation of the reconstruction data, a second algorithm employing \gls{drl} is used to obtain $\bm{\hat{\gamma}}$ from the initial estimate $\bm{\bar\gamma}$. The authors perform a comparison of \gls{psnr} with another residual sparse data reconstruction network called ReconNet \citep{7780424}. \han{The algorithm demonstrates improved \gls{psnr} and faster reconstruction than ReconNet.}


\begin{figure}[h]
\label{fig_unfolding}
\centering
\includegraphics[scale=0.5]{images/sparse_reconstruction.pdf}
\caption{\centering Inversion through unfolding of classical algorithms (left) or direct replacement via neural networks (right)}
\end{figure}
 
\han{In this study, researchers address artifact removal in initial reconstructions using \glspl{gan}\citep{8417964}.} As known, \glspl{gan} have two different network structures, one generates data and the other discriminates whether the data belongs to the labeled data or was transferred from the generator network. This process continues until the discriminator network starts to fail to differentiate between those two groups. In the paper, the initial data feeding generator network is obtained as ${\boldsymbol{\bar{\gamma}}} = \bm{G}^\dag\bm{p}_{\mathrm{rec}}$ where $\dag$ represents the pseudo-inverse. As a generator network, a deep residual network (ResNet) \citep{he2016deep} architecture is employed while the discriminator uses a \gls{cnn} architecture to classify between two groups of images. Additionally, between the generator and discriminator networks, another block is located which tunes the output of the generator network in order to generate a feasible set of images instead of overemphasizing the noise values of the pixels. \cy{Is it possible to quantify the performance of the GAN or even compare it to similar methods?}

\input{shrink_ultrasound/3.1.2_model_based_DL}

\input{shrink_ultrasound/3.2_tomography}

\input{sections/us_classification}

\subsection{Dictionary Learning} \label{sec:ut_dictlearning}
\han{(This is the modified and shrunken version.)}

In \han{ultrasound imaging inverse problems}, selecting an appropriate dictionary \cy{why and what is a dictionary in this context?} for the input data is \han{crucial}. This can be addressed \han{either} by reducing the mutual coherence of the dictionary matrix, or \han{through} standard optimization or learning techniques.  \cy{what problem does dictionary learning adress?}

\han{The $k$-SVD \citep{1710377}, a prominent method for dictionary optimization, is based on \gls{svd}}. it employs an alternating minimization approach, updating one dictionary matrix \han{column} and one data matrix \han{row} sequentially, while keeping \han{other} variables fixed. \han{Notably}, $k$-SVD employs an approximate error matrix for updating the column of the dictionary matrix, rather than the actual one. In the study \citep{Song2022}, \han{this limitation is addressed in sparsifying ultrasound elastography images by using the first principal component from the actual error matrix's \gls{pca}, in contrast to the $k$-SVD's use of the approximate error matrix's \gls{svd}.}  

Wavelet-based representation of the image is common in \gls{uct} and \gls{mri}, \han{but the search for a more suitable dictionary is ongoing} since those reconstructed images are not in the category of natural images.\cy{what is meant by natural images, and why is it important?} In \citep{tovsicultrasound}, authors \han{explore} a better dictionary representation for ultrasound tomography and \gls{mri} other than wavelet-based representation. They employ an optimization method \han{from} \citep{olshausen1996emergence}, which is an iterative alternating minimization method \han{minimizing} the loss function of the basis pursuit denoising problem.\cy{is this the adressed main problem adressed with dictionary learning?} \han{This method alternates between fixing the dictionary matrix and the image data, resulting in a 2dB improvement in \gls{psnr} level}\cy{is this a significant improvement?}.

\input{sections/SyntheticUS}

==> tikz_tables/fig_overview2.tex <==
\begin{tikzpicture}
    %======= Left ========
    %---- Inverse problem
    \draw \largeellipse{0, 10};
    \node[font=\huge] at (0, 12) {Inverse problems};
    \node [font=\Large] at (0, 10) {
        \begin{tabular}{cll}
            $\bullet$ & Denoising & ...\\
            $\bullet$ & Parameter recovery & \ref{sec:eddy_current}, \ref{sec:3ma2}, \ref{sec:3max8}\\
            $\bullet$ & Imaging & \ref{model_based_DL}, \ref{section_tomography}\\
            $\bullet$ & Beamforming & \ref{model_based_DL}\\
            %$\bullet$ & Compressed sensing & ...\\
        \end{tabular}
    };		
    
    %---- Forward problem
    \draw \mediumellipse{5.5, 4.5};
    \node[font=\huge] at (5.5, 5.5) {Forward problems};
    \node [font=\Large] at (5.5, 4.0) {
        \begin{tabular}{cll}
            $\bullet$ & Solving PDEs & \ref{section_tomography}\\
            $\bullet$ & Data synthesization & ...\\
        \end{tabular}
    };	
    \node [font=\Large] at (5.5, 3.0) {
        \begin{tabular}{cl}
            Refs: & \citep{Karniadakis21pinnreview}, \citep{raissi2019physics} \\
        \end{tabular}
    };
    
    %---- Dictionary learning
    \draw \smallellipse{0, 0.0};
    \node[font=\huge] at (0, 0.5) {Dictionary learning};
    \node [font=\Large] at (0, -0.5) {
        \begin{tabular}{cll}
            $\bullet$ & Optimal sensor excitation & ...\\
        \end{tabular}
    };		
    
    %======= Right ========
    %---- Covariance estimation
    \draw \mediumellipse{21.5, 11};
    \node[font=\huge] at (21.5, 12.5) {Information maximization};
    \node [font=\Large] at (21.0, 11) {
        \begin{tabular}{cll}
            $\bullet$ & Sensor placement & ...\\
            $\bullet$ & Optimal sensor excitation & ...\\ 
        \end{tabular}
    };		
    
    %---- Metric learning
    \draw \largeellipse{17.5, 5.5};
    \node[font=\huge] at (16.0, 7.0) {Metric learning};
    \node [font=\Large] at (17.0, 5.0) {
        \begin{tabular}{cll}
            $\bullet$ & Detection & \ref{opt._insp.}\\
            $\bullet$ & Classification & \ref{us_classification} \\
            $\bullet$ & Localization / segmentation & \ref{opt._insp.}\\
        \end{tabular}
    };		
    
    %---- Dimensionality reduction
    \draw \mediumellipse{21, 0.0};
    \node[font=\huge] at (21, 0.5) {Dimensionality reduction};
    \node [font=\Large] at (21, -1.0) {
        \begin{tabular}{cll}
            $\bullet$ & Feature extraction & \ref{opt._insp.}\\
            $\bullet$ & Subspace projection & \ref{sec:pct}\\
            $\bullet$ & Manifold learning & \\
        \end{tabular}
    };		
\end{tikzpicture}
